Design and Implementation of the New D0 Level-1 Calorimeter Trigger

Increasing luminosity at the Fermilab Tevatron collider has led the D0 collaboration to make improvements to its detector beyond those already in place for Run IIa, which began in March 2001. One of the cornerstones of this Run IIb upgrade is a completely redesigned level-1 calorimeter trigger system. The new system employs novel architecture and algorithms to retain high efficiency for interesting events while substantially increasing rejection of background. We describe the design and implementation of the new level-1 calorimeter trigger hardware and discuss its performance during Run IIb data taking. In addition to strengthening the physics capabilities of D0, this trigger system will provide valuable insight into the operation of analogous devices to be used at LHC experiments.

==> Makefile <==
#----------------------------------------------------
# Generic make file for LaTeX: requires GNU make
#
# This makefile provides four targets: dvi, pdf and clean.
# The default is "pdf".
# To make a dvi file, type "make dvi"
# To make a pdf file, type "make pdf" or simply "make".
# To remove all files generated by make, type "make clean".
#
# original from:
# Rouben Rostmaian <rostamian@umbc.edu>
# September 2002
# http://www.math.umbc.edu/~rouben/prosper/large_sample/Makefile
#
# Modifications
# 03-Apr-07  add LATEX and DVIPDF
#-------------------------------------------------------

TEXFILE	= l1cal2b_nim.tex
LATEX   = latex
DVIPDF  = dvipdfm

.PHONY: dvi pdf

pdf:	$(TEXFILE:.tex=.pdf)
dvi:	$(TEXFILE:.tex=.dvi)

%.dvi: %.tex
	${LATEX} $<
	latex_count=5 ;\
	while grep 'Rerun to get cross-references right' $(TEXFILE:.tex=.log) && [ $$latex_count -gt 0 ] ;\
		do \
			${LATEX} $< ;\
			latex_count=`expr $$latex_count - 1` ;\
		done

%.pdf: %.dvi
	${DVIPDF} -o $(<:.dvi=.pdf) $<

clean:
	@rm -f \
	$(TEXFILE:.tex=.aux) \
	$(TEXFILE:.tex=.log) \
	$(TEXFILE:.tex=.out) \
	$(TEXFILE:.tex=.dvi) \
	$(TEXFILE:.tex=.pdf)

# DO NOT DELETE



